Parallel Graph Algorithms in Constant Adaptive Rounds: Theory meets Practice

We study fundamental graph problems such as graph connectivity, minimum spanning forest (MSF), and approximate maximum (weight) matching in a distributed setting. In particular, we focus on the Adaptive Massively Parallel Computation (AMPC) model, which is a theoretical model that captures MapReduce-like computation augmented with a distributed hash table. We show the first AMPC algorithms for all of the studied problems that run in a constant number of rounds and use only $O(n^\epsilon)$ space per machine, where $0 < \epsilon < 1$. Our results improve both upon the previous results in the AMPC model, as well as the best-known results in the MPC model, which is the theoretical model underpinning many popular distributed computation frameworks, such as MapReduce, Hadoop, Beam, Pregel and Giraph. Finally, we provide an empirical comparison of the algorithms in the MPC and AMPC models in a fault-tolerant distriubted computation environment. We empirically evaluate our algorithms on a set of large real-world graphs and show that our AMPC algorithms can achieve improvements in both running time and round-complexity over optimized MPC baselines.

==> inputs/forest.tex <==
\section{Improved Forest Connectivity}\label{sec:forest}

\newcommand{\shrink}[0]{\textsc{Shrink}}

In this section we show how to find the connected components problem in a graph, whose each connected component is a tree.
In~\cite{AMPC} it was shown that the problem can be solved in $O(1)$ AMPC rounds using $O(n \log n)$ queries.
Here we show that the query complexity can be improved to $O(n \log \log n)$.

The algorithm begins by transforming each tree to a cycle of asymptotically the same size using an Euler-Tour tree.
This is a standard reduction which takes only $O(1)$ rounds and $O(n)$ space (see~\cite{AMPC} for details).

In the following steps we use the \shrink procedure, whose pseudocode is given below.

\begin{tboxalg}{$\shrink(G=(V, E), p)$}\label{alg:shrink}
        \begin{enumerate}[ref={\arabic*-}, topsep=0pt,itemsep=0ex,partopsep=0ex,parsep=1ex, leftmargin=*]
        \item Sample each vertex independently with probability $p$.
                Denote the set of sampled vertices by $M$.
          Randomly distribute the vertices of $M$ to the machines.

  \item \label{alg:step2} For each sampled vertex $v$ traverse the cycle in each direction
        until a sampled vertex is reached. Let $l_v$ and $r_v$ be the sampled vertices,
                                        where the each of two traversals finishes.

    \item Return the graph $(M, \{xl_x \mid x \in M\} \cup \{xr_x \mid x \in M\})$.
  \end{enumerate}
\end{tboxalg}

\begin{lemma}\label{lem:shrink}
Let $G$ be an $n$-vertex graph consisting of cycles and $0 < p \leq 1$.
Consider a cycle of $G$ of length $k \geq 1/p$.
Then, $\shrink(G, p)$ shrinks the cycle by a factor of $\Omega(1/p)$ with probability $1 - \exp(\Omega(k/p))$.
Moreover, the longest traversed part of a cycle in step~\ref{alg:step2} is $t/p$ with probability $1-n\exp(-\Omega(t/p))$.
\end{lemma}

\begin{proof}
By Chernoff bound, the number of sampled points on a cycle of length $k \geq 1/p$ is $\Theta(k/p)$ with probability $1 - \exp(-\Omega(k/p))$.
Note that the number of sampled points is also the number of points in the resulting cycle.

The algorithm traverses a fixed segment of length $t/p$ if none of the $t/p-2$ vertices within the segment are sampled.
This happens with probability $(1-1/p)^{t/p-2} = \exp(-\Omega(t))$.
Since there are at most $n$ segments to consider, we obtain the desired by taking union bound.
\end{proof}

The complete algorithm for forest connectivity is given below.
\begin{tboxalg}{$\textsc{ForestConnectivity}(G)$}\label{alg:fc}
        \begin{enumerate}[ref={\arabic*-}, topsep=0pt,itemsep=0ex,partopsep=0ex,parsep=1ex, leftmargin=*]

        \item For $i := 1, \ldots, 3/\epsilon$:
                        \begin{enumerate}[ref={(\alph*)}, topsep=5pt,itemsep=0ex]		\item $G := \shrink{}(G, n^{-\epsilon/2})$.
	\end{enumerate}
	\item $G := \shrink{}(G, 1/\log n)$
  \item
  \end{enumerate}
\end{tboxalg}

\begin{theorem}
There exists an AMPC algorithm that solves the forest connectivity problem in $O(1)$ rounds using $T = O(n \log \log n)$ total space w.h.p.
\end{theorem}

\begin{proof}
The first $O(1/\epsilon)$ calls to $\shrink{}(G, n^-{\epsilon/2})$ $O(1/\epsilon)$ shrink the longest cycle to have size $O(n^\epsilon)$.
This happens by high probability by Lemma~\ref{lem:shrink}.
Then, $\shrink{}(G, 1/log n)$ shrinks each cycle of length $\Omega(\log^2 n)$ by a factor of $\Omega(\log n)$.

Assume that among the $n$ vertices of the original graph there are $l$ vertices in long cycles, that is of length $\Omega(\log^2 n)$, and the remaining $s = n -l$ vertices are in short cycles.

After the calls to shrink, the number of vertices in long cycles is at most $l/\log n$ and each cycle has length $O(n^\epsilon)$.

The forest connectivity algorithm of~\cite{AMPC} takes $O(1)$ rounds and in expectation uses $O(\log k)$ queries for a cycle of length $k$.

Hence the expected number of queries made after our preprocessing is
\[
	(l/\log n) O(\log n) + (n-l) \log O(\log^2 n) = l + (n-l) O(\log \log n) = O(n \log \log n)
\]

TODO: show a whp bound on the number of queries.
\end{proof}


==> inputs/prelims.tex <==
\section{Preliminaries}
We denote an unweighted graph by $G(V, E)$, where $V$ is the set of
vertices and $E$ is the set of edges in the graph. The number of
vertices in a graph is $n = |V|$, and the number of edges is $m =
|E|$. We assume vertices are indexed from $0$ to $n-1$.  We assume
that there are no self-edges or duplicate edges in the graph.
We say that an algorithm has $O(f(n))$ cost \emph{with high
probability (w.h.p.)} if it has $O(k\cdot f(n))$ cost with probability
at least $1 - 1/n^{k}$.

In the descriptions of our algorithms we highlight the parts which
rely on \AMPC{} model features. The remaining parts can be
implemented in \MPC{} model using standard primitives, such as
sorting, duplicate removal, etc, all of which run in space
proportional to the input and $O(1/\epsilon)$ rounds of both \MPC{}
and \AMPC{} computation.



==> inputs/queries.tex <==
\begin{table}[!t]
\footnotesize
\centering
\begin{tabular}[t]{l | c | c }
  \toprule
  {\bf Graph} &  \multicolumn{1}{c|}{\bf \AMPC{}-MIS-(NC)} & \multicolumn{1}{c}{\bf \AMPC{}-MIS(C)} \\
  \midrule
  2x100M            & 200M   & 200M  \\
  2x1B              & 2B     & 2B    \\
  2x10B             & 20B    & 20B   \\
  com-Orkut         & 155M   & 74.3M \\
  Friendster        & 2.61B  & 1.49B \\
  ClueWeb           & 37.2B  & 10.4B \\
\end{tabular}
\caption{\small
This table reports the number of queries issued by the \AMPC{}-MIS algorithm without caching (NC) and with caching (C) for a subset of our graph inputs.
  \label{table:queries}
\end{table}

